A link invariant related to Khovanov homology and knot Floer homology

In this paper we introduce a chain complex $C_{1 \pm 1}(D)$ where D is a plat braid diagram for a knot K. This complex is inspired by knot Floer homology, but it the construction is purely algebraic. It is constructed as an oriented cube of resolutions with differential d=d_0+d_1. We show that the E_2 page of the associated spectral sequence is isomorphic to the Khovanov homology of K, and that the total homology is a link invariant which we conjecture is isomorphic to \delta-graded knot Floer homology. The complex can be refined to a tangle invariant for braids on 2n strands, where the associated invariant is a bimodule over an algebra A_n. We show that A_n is isomorphic to B'(2n+1, n), the algebra used for the DA-bimodule constructed by Ozsvath and Szabo in their algebraic construction of knot Floer homology.

==> algebras.tex <==
\section{OS algebra}
To a collection of $2n$ points we can associate two algebras over $\mathbb{F}[U_1,...,U_{2n}]$ denoted by $A_n$ (our algebra) and $\mathcal{C}(n)=\mathcal{B}(2n,n)$ (I think).

Let us first review the definition of $\mathcal{C}(n)$ (This is the algebra that Zoltan defined in his course).
A \emph{local state} is a subset $\x\subset \{1+1/2,2+1/2...,2n-1/2\}$ of $n$ elements, or equivalently a choice of $n$ closed intervals of the form $[i,i+1]$. For each local state $\x$ there is an idempotent denoted by $I_{\x}$ in $\mathcal{C}(n)$. Also, $\mathcal{C}(n)$ contains generators $R_i$ and $L_i$ for shifting to the right and left, respectively. 

Multiplication rule: For idempotents $I_{\x}$ that $i-1/2\in\x$ and $i+1/2\notin\x$ we have $I_{\x}R_iL_i=U_iI_\x$, otherwise $I_{\x}R_iL_i=0$. Similarly if $i+1/2\in\x$ and $i-1/2\notin\x$ then $I_{\x}L_iR_i=U_iI_x$, otherwise $I_{\x}L_iR_i=0$. 

Rules:
\begin{enumerate}
\item $R_iR_{i+1}=0$ and $L_{i+1}L_{i}=0$ for all $i$.
\item If $\{i-1/2,i+1/2\}\cap\x=\emptyset$, then $U_iI_{\x}=0$.
\end{enumerate}

For each local state $\x$ there is subset $S_{\x}\subset\{1,2,...,2n\}$ defined as 
\[S_{\x}=\{1\}\cup\{i\ |\ i-1/2\notin \x\}.\]
Therefore, each idempotent $I_{\x}\in\mathcal{C}(n)$ identifies an idempotent in $A_n$. Furthermore, under this identification $R_i$ and $L_i$ in $\mathcal{C}(n)$ correspond to $L_i$ and $R_i$ in $A_n$, respectively. 

Observations:

\begin{itemize}
\item[-] Multiplication: If $\{i-1/2,i+1/2\}\cap \x=\{i-1/2\}$, then $\{i,i+1\}\cap S_{\x}=\{i+1\}$, and so $\iota_{S_{\x}}L_iR_i=U_i\iota_{S_{\x}}$. Similarly, if $\{i-1/2,i+1/2\}\cap \x=\{i+1/2\}$, then $\{i,i+1\}\cap S_{\x}=\{i\}$ and so $\iota_{S_{\x}}R_iL_i=U_i\iota_{S_{\x}}$. Also, if $\{i-1/2,i+1/2\}\subset \x$ then $\{i,i+1\}\cap S_{\x}=\emptyset$. Thus, $\iota_{S_{\x}}R_iL_i=\iota L_iR_i=0$, while $U_i\iota_{S_{\x}}\neq 0$.
\item[-] Rule 2: If $\{i-1/2,i+1/2\}\cap \x=\emptyset$, then $\{i,i+1\}\subset S_{\x}$ and thus $U_i\iota_{S_{\x}}=\iota_{S_{\x}}R_iL_i=0$.
\item[-] Rule 1: Suppose $\x$ is a local state such that $R_iR_{i+1}I_{\x}$ would be nonzero if we don not have Rule $1$ i.e. $\{i-1/2,i+1/2,i+3/2\}\cap\x=\{i+3/2\}$. Then, $S_{\x}\cap \{i,i+1,i+2\}=\{i,i+1\}$. Then, $L_iL_{i+1}\iota_{S_{\x}}\neq 0$ with our relations, but we prove that for any cycle $Z$ in an upper half singular braid $B$ if $\{i,i+1\}\subset b(Z)$ then $L_iL_{i+1}x_Z=0$. To prove this we use induction and prove that if $\{i,i+1,...,j\}\cap b(Z)=\{i,j\}$ then $L_{j-1}L_{j-2}...L_iL_{j}x_Z=0$ for all $i$ and $j$. Similarly, if $b(Z)\cap\{i,i+1,i+2\}=\{i+1,i+2\}$ then $R_{i+1}R_ix_Z=0$.



\end{itemize}








